Incremental Multi-Scene Modeling via Continual Neural Graphics Primitives

Neural radiance fields (NeRF) have revolutionized photorealistic rendering of novel views for 3D scenes. Despite their growing popularity and efficiency as 3D resources, NeRFs face scalability challenges due to the need for separate models per scene and the cumulative increase in training time for multiple scenes. The potential for incrementally encoding multiple 3D scenes into a single NeRF model remains largely unexplored. To address this, we introduce Continual-Neural Graphics Primitives (C-NGP), a novel continual learning framework that integrates multiple scenes incrementally into a single neural radiance field. Using a generative replay approach, C-NGP adapts to new scenes without requiring access to old data. We demonstrate that C-NGP can accommodate multiple scenes without increasing the parameter count, producing high-quality novel-view renderings on synthetic and real datasets. Notably, C-NGP models all $8$ scenes from the Real-LLFF dataset together, with only a $2.2\%$ drop in PSNR compared to vanilla NeRF, which models each scene independently. Further, C-NGP allows multiple style edits in the same network.

==> section/00_abstract.tex <==
\begin{abstract}
Neural radiance fields (NeRF) have revolutionized photorealistic rendering of novel views for 3D scenes. Despite their growing popularity and efficiency as 3D resources, NeRFs face scalability challenges due to the need for separate models per scene and the cumulative increase in training time for multiple scenes. The potential for incrementally encoding multiple 3D scenes into a single NeRF model remains largely unexplored. To address this, we introduce Continual-Neural Graphics Primitives (C-NGP), a novel continual learning framework that integrates multiple scenes incrementally into a single neural radiance field. Using a generative replay approach, C-NGP adapts to new scenes without requiring access to old data. We demonstrate that C-NGP can accommodate multiple scenes without increasing the parameter count, producing high-quality novel-view renderings on synthetic and real datasets. Notably, C-NGP models all $8$ scenes from the Real-LLFF dataset together, with only a $2.2\%$ drop in PSNR compared to vanilla NeRF, which models each scene independently. Further, C-NGP allows multiple style edits in the same network. The code, implementation details, and dynamic visualizations are in the supplementary material.
\end{abstract}

==> tables/ablationcomp.tex <==
% \begin{table}[!t]
% \centering
% \resizebox{\linewidth}{!}{
% \def\arraystretch{1.1}
% \begin{tabular}{c|ccc}
% \hline
% Experiments                              & PSNR $\uparrow$
%  & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ \hline
% XYZ | C + $SE(\theta, \phi)$                                 & 24.108                        & 0.812                          & 0.201                            \\
% XYZ + $\psi(C)$ + $SE(\theta, \phi)$                            & 12.966                        & 0.813                          & 0.460                            \\
% XYZ | C + $\psi(C)$ + $SE(\theta, \phi)$          & 24.492                        & 0.824                          & 0.184                            \\ 
% XYZ | C + $\psi(C)$ + $SE(\theta, \phi)$ + $\psi(C)$               & \cellcolor[HTML]{D0E0E3}\textbf{25.927} & \cellcolor[HTML]{D0E0E3}\textbf{0.880} & \cellcolor[HTML]{D0E0E3}\textbf{0.139} \\ \hline
% \end{tabular}}
% \caption{Ablation on the configuration choice for conditioning Instant-NGP network \cite{muller2022instant} - the backbone of C-NGP.}
% \label{table:ablation}
% \vspace{-3mm}
% \end{table}

==> tables/nerfsynthcomp.tex <==
% \begin{table}[!t]
% \resizebox{\linewidth}{!}{
% \def\arraystretch{1.0}%
% \begin{tabular}{c|c|ccc}
% \hline
%                                             &                                                                                  & \multicolumn{3}{c}{NeRF Synthetic 360$^{\circ}$}                                                                            \\ \cline{3-5} 
% \multirow{-2}{*}{Method}                    & \multirow{-2}{*}{Finetuning}                                                      & PSNR $\uparrow$                                 & SSIM $\uparrow$                                 & LPIPS $\downarrow$                               \\ \hline
% % \multicolumn{1}{c|}{NeRF*}                   & x                                                                              & 25.31                                  & 0.87                                  & 0.16                                  \\
% \multicolumn{1}{c|}{NeRF*}                   & x                                                                              & 21.75                                 & 0.84                                  & 0.16                                  \\
% \multicolumn{1}{c|}{IBRNet \cite{wang2021ibrnet}}                 & \checkmark                                                                          & 28.14                                  & 0.94                                  & 0.07                                  \\
% \multicolumn{1}{c|}{MVSNeRF \cite{chen2021mvsnerf}}                & \checkmark                                                                          & 27.07                                  & 0.93                                  & 0.17                                  \\
% \multicolumn{1}{c|}{CP-NeRF \cite{he2023cp}}                & x                                                                              & \textbf{29.54 }                                 & 0.92                                  & 0.09                                  \\
% \multicolumn{1}{c|}{\textbf{C-NGP (ours)}} & x                                                                              & 29.40          & \textbf{0.94} & \textbf{0.09} \\ \hline
% \multicolumn{1}{c|}{CP-NeRF \cite{he2023cp}}                & \checkmark                                                                          & 31.77                                  & 0.95                                  & 0.06                                  \\
% \multicolumn{1}{c|}{\textbf{C-NGP (ours)}} & \checkmark                                                                          & \textbf{32.08} & \textbf{0.95} & \textbf{0.06} \\ \hline
% \end{tabular}}
% \caption{Quantitative comparison on NeRF Synthetic $360^{\circ}$ dataset \cite{mildenhall2021nerf} across different baseline methods. Our continual framework shows competitive performance with multi-scene modeling and even outperforms the previous state-of-the-art methods. NeRF* indicates vanilla NeRF trained under the proposed continual setup.}
% \label{table:nerf_synth}
% % \vspace{-3mm}
% \end{table}

==> tables/offline_online_sampling.tex <==
% \begin{table}[!t]
% \resizebox{\linewidth}{!}{
% \def\arraystretch{1.7}%
% \begin{tabular}{c|ccc|ccc}
% \hline
%                                              & \multicolumn{3}{c|}{Offline Sampling}                                                         & \multicolumn{3}{c}{Online Sampling}                                                           \\ \cline{2-7} 
% \multirow{-2}{*}{Datasets}                   & PSNR $\uparrow$                           & SSIM $\uparrow$                        & LPIPS $\downarrow$                         & PSNR  $\uparrow$                         & SSIM $\uparrow$                        & LPIPS $\downarrow$                        \\ \hline
% \multicolumn{1}{c|}{NeRF Synthetic 360$^{\circ}$} & 25.211                         & 0.86                         & 0.151                         & 29.40                          & 0.93                         & 0.09                          \\
% \multicolumn{1}{c|}{Blender Synthetic}   & 37.735 & 0.98 & 0.022 & 37.734 & 0.98 & 0.022 \\ \hline
% \end{tabular}}
% \caption{Offline vs Online sampling strategy. Analyzing the quantitative performance on training with the available training data (offline) or through images generated through the generative replay (online) while learning C-NGP. The enhanced performance with online sampling is due to the same camera parameters across all the scenes.}
% \label{table:samplingmethod}
% \end{table}
